Sparsification Lower Bound for Linear Spanners in Directed Graphs

For $\alpha \ge 1$, $\beta \ge 0$, and a graph $G$, a spanning subgraph $H$ of $G$ is said to be an $(\alpha, \beta)$-spanner if $\dist(u, v, H) \le \alpha \cdot \dist(u, v, G) + \beta$ holds for any pair of vertices $u$ and $v$. These type of spanners, called \emph{linear spanners}, generalizes \emph{additive spanners} and \emph{multiplicative spanners}. Recently, Fomin, Golovach, Lochet, Misra, Saurabh, and Sharma initiated the study of additive and multiplicative spanners for directed graphs (IPEC $2020$). In this article, we continue this line of research and prove that \textsc{Directed Linear Spanner} parameterized by the number of vertices $n$ admits no polynomial compression of size $\calO(n^{2 - \epsilon})$ for any $\epsilon > 0$ unless $\NP \subseteq \coNP/poly$. We show that similar results hold for \textsc{Directed Additive Spanner} and \textsc{Directed Multiplicative Spanner} problems. This sparsification lower bound holds even when the input is a directed acyclic graph and $\alpha, \beta$ are \emph{any} computable functions of the distance being approximated.

==> abstract.tex <==
For $\alpha \ge 1$, $\beta \ge 0$,  and a graph $G$, a spanning subgraph $H$ of $G$ is said to be an $(\alpha, \beta)$-spanner if $\dist(u, v, H) \le \alpha \cdot \dist(u, v, G) + \beta$ holds for any pair of vertices $u$ and $v$.
These type of spanners, called \emph{linear spanners},  generalizes additive spanners and multiplicative spanners.
Recently,  Fomin,  Golovach,  Lochet,  Misra,  Saurabh,  and Sharma initiated the study of additive and multiplicative spanners for directed graphs (IPEC $2020$).
In this article,  we continue this line of research and prove that  \textsc{Directed Linear Spanner} parameterized by the number of vertices $n$ admits no generalized kernel of size $\calO(n^{2 - \epsilon})$ for any $\epsilon > 0$ unless $\NP \subseteq \coNP/poly$.
With some simple modifications, we can show that similar results hold for \textsc{Directed Additive Spanner} and \textsc{Directed Multiplicative Spanner} problems.
This sparsification lower bound holds even when input is a directed acyclic graph and $\alpha,  \beta$ are sub-polynomial in $n$.
